Unsupervised Learning for Solving the Travelling Salesman Problem

We propose UTSP, an unsupervised learning (UL) framework for solving the Travelling Salesman Problem (TSP). We train a Graph Neural Network (GNN) using a surrogate loss. The GNN outputs a heat map representing the probability for each edge to be part of the optimal path. We then apply local search to generate our final prediction based on the heat map. Our loss function consists of two parts: one pushes the model to find the shortest path and the other serves as a surrogate for the constraint that the route should form a Hamiltonian Cycle. Experimental results show that UTSP outperforms the existing data-driven TSP heuristics. Our approach is parameter efficient as well as data efficient: the model takes $\sim$ 10\% of the number of parameters and $\sim$ 0.2\% of training samples compared with reinforcement learning or supervised learning methods.

==> Figures/donut.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Donut [id:dp8164065064704229] 
\draw   (145.86,196.62) .. controls (119.29,187.99) and (104.74,159.44) .. (113.38,132.86) .. controls (122.01,106.29) and (150.56,91.74) .. (177.14,100.38) .. controls (203.71,109.01) and (218.26,137.56) .. (209.62,164.14) .. controls (200.99,190.71) and (172.44,205.26) .. (145.86,196.62)(122.41,268.81) .. controls (55.96,247.22) and (19.6,175.85) .. (41.19,109.41) .. controls (62.78,42.96) and (134.15,6.6) .. (200.59,28.19) .. controls (267.04,49.78) and (303.4,121.15) .. (281.81,187.59) .. controls (260.22,254.04) and (188.85,290.4) .. (122.41,268.81) ;
%Straight Lines [id:da08537551182138348] 
\draw    (191.24,189.44) -- (235.85,250.84) ;

%Straight Lines [id:da834216281810359] 
\draw    (161.5,22) -- (161.5,97.9) ;
%Straight Lines [id:da5206227009363016] 
\draw    (281.81,109.41) -- (209.62,132.86) ;
%Straight Lines [id:da8445125715568087] 
\draw    (87.15,250.84) -- (131.76,189.44) ;
%Straight Lines [id:da024670712821340035] 
\draw    (41.19,109.41) -- (113.38,132.86) ;




\end{tikzpicture}


==> Tables/NewNeuripsTable3.tex <==
% \onecolumn
\begin{table*}[t]
\small
\centering
\caption{Results of SAG + Local Search w.r.t. existing baselines. We evaluate the models on 128 TSP 500 instances and 128 TSP 1000 instances.}
\vskip 0.15in
\label{table:Exps03}
\begin{tabular}{llllllll}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Type} & \multicolumn{3}{c}{TSP500} & \multicolumn{3}{c}{TSP1000} \\
 & & Length & Gap (\%) & Time & Length & Gap (\%) & Time \\
\hline
Concorde & Solver & 16.55 & 0.00 & 37.66m & 23.12 & 0.00 & 6.65h \\
Gurobi & Solver & 16.52 & -0.17 & 45.63h & - & - & - \\
LKH3 & Heuristic & 16.55 & 0.00 & 11.41m & 23.12 & 0.00 & 38.09m \\
GAT \cite{deudon2018learning} & RL, S & 28.63 & 73.03 & 20.18m & 50.30 & 117.59 & 37.07m \\
GAT \cite{deudon2018learning} & RL, S 2-OPT & 23.75 & 43.57 & 57.76m & 47.73 & 106.46 & 5.39h \\
GAT \cite{kool2018attention} & RL, S & 22.64 & 36.84 & 15.64m & 42.80 & 85.15 & 63.97m \\
GAT \cite{kool2018attention} & RL, G & 20.02 & 20.99 & 1.51m & 31.15 & 34.75 & 3.18m \\
GAT \cite{kool2018attention} & RL, BS & 19.53 & 18.03 & 21.99m & 29.90 & 29.24 & 1.64h \\
GCN \cite{joshi2019efficient} & SL, G & 29.72 & 79.61 & 6.67m & 48.62 & 110.29 & 28.52m \\
GCN \cite{joshi2019efficient} & SL, BS & 30.37 & 83.55 & 38.02m & 51.26 & 121.73 & 51.67m \\
GCN \cite{joshi2019efficient} & SL, BS* & 30.43 & 83.89 & 30.62m & 51.10 & 121.04 & 3.23h \\
\hline
Att-GCRN \cite{fu2021generalize} & SL+RL MCTS & 16.75 & 1.22 & 31.17s + 3.33m & 23.52 & 1.72 & 43.94s + 6.68m \\
\hline
\textbf{UTSP (Ours)} & UL, Search & 16.68 & \textbf{0.84} & 1.37m + 1.33m & 23.39 & \textbf{1.18} & 3.35m + 2.67m \\
\bottomrule
\end{tabular}
\end{table*}
% \twocolumn

==> Tables/TSPperformance.tex <==
% \onecolumn
\begin{table*}[htb]
\footnotesize
\centering
\caption{Results of SAG + Local Search  w.r.t. existing baselines, tested on 10,000 instances with $n$ = 20, 50 and 100.}
%\Yiwei{[Yiwei: I keep the two results here only for comparison, I think finally we only keep the best one. I did not tune too much parameters (2 - 4 sets for each TSP variant). I would like to tune and search a longer one for TSP10000.]}
\vskip 0.15in
\label{table:Exps01}
    \begin{tabular}{lllllllllll}
    \toprule
    %   \toprule[2pt]
       \multirow{2}{*}{Method} & \multirow{2}{*}{Type}  & \multicolumn{3}{c}{TSP20} & \multicolumn{3}{c}{TSP50} & \multicolumn{3}{c}{TSP100}\\
         &  & Length & Gap (\%)  & Time & Length & Gap (\%) & Time & Length & Gap (\%)  & Time \\
        \hline
        Concorde  & Solver & {3.8303} & {0.0000 } & {2.31m} & {5.6906} & {0.0000 } & {13.68m} & {7.7609} & {0.0000 } & {1.04h}  \\
        Gurobi  & Solver & {3.8302} & {-0.0001 } & {2.33m} & {5.6905} & {0.0000 } & {26.20m} & {7.7609} & {0.0000 } & {3.57h}  \\
        LKH3  & Heuristic & {3.8303} & {0.0000 } & {20.96m} & {5.6906} & {0.0008 } & {26.65m} & {7.7611} & {0.0026 } & {49.96m}  \\
        % \hline
         GAT \citep{deudon2018learning}  & RL, S &  {3.8741} &  {1.1443 } &   {10.30m} &  {6.1085} &  {7.3438 } &   {19.52m} &  {8.8372} &  {13.8679 } &   {47.78m}  \\

        GAT \citep{deudon2018learning}  & \tabincell{c}{RL, S\\ 2-OPT} &  {3.8501} &  {0.5178 } &  {15.62m} & {5.8941} & {3.5759 } & {27.81m} & {8.2449} & {6.2365 } & {4.95h}  \\

        GAT \citep{kool2018attention}  & RL, S &  {3.8322} &  {0.0501 } &   {16.47m}  & {5.7185} & {0.4912 } &  {22.85m} & {7.9735} & {2.7391 } & {1.23h}  \\

        GAT \citep{kool2018attention}  & RL, G & {3.8413} & {0.2867 } & {6.03s} & {5.7849} & {1.6568 } & {34.92s} & {8.1008} & {4.3791 } & {1.83m} \\

        GAT \citep{kool2018attention}  & RL, BS &  {3.8304} &  {0.0022 } &  {15.01m} & {5.7070} & {0.2892 } & {25.58m} & {7.9536} & {2.4829 } & {1.68h}  \\

        GCN \citep{joshi2019efficient} & SL, G & {3.8552} & {0.6509 } &  {{19.41s}} & {5.8932} & {3.5608 } &  {2.00m} & {8.4128} & {8.3995 } &  {11.08m}  \\

        GCN \citep{joshi2019efficient} & SL, BS &  {3.8347} &  {0.1158 } &   {21.35m} &  {5.7071} &  {0.2905 } &   {35.13m} &  {7.8763} &  {1.4828 } &   {31.80m}  \\

        GCN \citep{joshi2019efficient} & SL, BS* & {3.8305} & {0.0075 } & {22.18m} & {5.6920} & {0.0251 } & {37.56m} & {7.8719} & {1.4299 } & {1.20h}  \\

        \hline
        \multirow{2}{*} {Att-GCRN\citep{fu2021generalize}} & \multirow{2}{*}{\tabincell{c}{SL+RL \\MCTS}} & \multirow{2}{*}{{3.8300}} & \multirow{2}{*}{\textbf{-0.0074}} & {23.33s} +  & \multirow{2}{*}{5.6908} & \multirow{2}{*}{{0.0032 }} & {2.59m} +  & \multirow{2}{*}{{7.7616}} & \multirow{2}{*}{{0.0096 }} & {3.94m} +   \\
        & & & & 1.05m & & & 2.63m & & & 5.25m\\ \hline

        % \multirow{2}{*} {\tabincell{c}{Random Init ($T = 0.01$)}} & \multirow{2}{*}{MCTS} & \multirow{2}{*}{{NA}} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{NA} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{{7.8752}} & \multirow{2}{*}{1.473 } & {0+}   \\
        % & & & & NA & & & NA & & & 6m\\     \hline
        %  \multirow{2}{*} {\tabincell{c}{Random Init ($T = 0.02$)}} & \multirow{2}{*}{MCTS} & \multirow{2}{*}{{NA}} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{NA} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{{7.8483}} & \multirow{2}{*}{1.126 } & {0+}   \\
        % & & & & NA & & & NA & & & 12m\\     \hline
        %   \multirow{2}{*} {\tabincell{c}{Uniform Init ($T = 0.01$)}} & \multirow{2}{*}{MCTS} & \multirow{2}{*}{{NA}} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{NA} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{{7.8332}} & \multirow{2}{*}{0.932 } & {0+}   \\
        % & & & & NA & & & NA & & & 6m\\     \hline     
        %   \multirow{2}{*} {\tabincell{c}{Uniform Init ($T = 0.02$)}} & \multirow{2}{*}{MCTS} & \multirow{2}{*}{{NA}} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{NA} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{{7.8084}} & \multirow{2}{*}{0.612 } & {0+}   \\
        % & & & & NA & & & NA & & & 12m\\     \hline
        %\usepackage{supertabular}??
        \multirow{2}{*} {{\bf{\small{UTSP} (ours)}} } & \multirow{2}{*}{UL, Search} & \multirow{2}{*}{{3.8303}} & \multirow{2}{*}{-0.0009} & {38.23s} +  & \multirow{2}{*}{5.6894} & \multirow{2}{*}{\textbf{-0.0200}} & {1.34m} +  & \multirow{2}{*}{{7.7608}} & \multirow{2}{*}{\textbf{-0.0011 }} & {5.68m+}   \\
        & & & & 1.04m & & & 2.60m & & & 5.21m\\ 
        % \multirow{1}{*} {\textbf{Ours (Restart)} ($T = 0.01$s)} & \multirow{1}{*}{UL, Search} & \multirow{1}{*}{{N/A}} & \multirow{1}{*}{\textbf{N/A}} & {38.23s} +  & \multirow{1}{*}{N/A} & \multirow{1}{*}{\textbf{-0.02}} & {1.34m} +  & \multirow{1}{*}{{7.760}} & \multirow{1}{*}{\textbf{-0.011 }} & {5.68m+}   \\
        % & & & & 1.04m & & & 2.60m & & & 5.21m\\ 
\bottomrule
        % \bottomrule[2pt]
    \end{tabular}
\end{table*}
% \twocolumn

==> Tables/TSPperformance2.tex <==
% \onecolumn
\begin{table*}[t]
\footnotesize
\centering
\caption{Results of SAG + Local Search w.r.t. existing baselines, tested on 128 instances with $n$ = 200, 500 and 1000.}
\vskip 0.15in
\label{table:Exps02}
    \begin{tabular}{lllllllllll}
    \toprule
    %   \toprule[2pt]
       \multirow{2}{*}{Method} & \multirow{2}{*}{Type}  & \multicolumn{3}{c}{TSP200} & \multicolumn{3}{c}{TSP500} & \multicolumn{3}{c}{TSP1000}\\
         &  & Length & Gap (\%)  & Time & Length & Gap (\%)  & Time & Length & Gap (\%) & Time \\
        \hline
                Concorde &Solver & {10.7191} & {0.0000 } & {3.44m} & {16.5458} & {0.0000 } & {37.66m} & {23.1182} & {0.0000 } & {6.65h} \\
        Gurobi &Solver & {10.7036} & {-0.1446 } & {40.49m} & {16.5171} & {-0.1733 } & {45.63h} & {-} & {-} & {-}  \\
        LKH3 & Heuristic & {10.7195} & {0.0040 } & {2.01m} & {16.5463} & {0.0029 } & {11.41m} & {23.1190} & {0.0036 } & {38.09m}  \\
        % \hline
        GAT \citep{deudon2018learning} & RL, S & {13.1746} & {22.9079 } &  {4.84m} & {28.6291} & {73.0293 } &  {20.18m} & {50.3018} & {117.5860 } & {37.07m}  \\

        GAT \citep{deudon2018learning} & \tabincell{c}{RL, S\\ 2-OPT} & {11.6104} & {8.3159 } & {9.59m} & {23.7546} & {43.5687 } & {57.76m} & {47.7291} & {106.4575 } & {5.39h}  \\

        GAT \citep{kool2018attention}  & RL, S & {11.4497} & {6.8160 } &  {4.49m} & {22.6409} & {36.8382 } & {15.64m} & {42.8036} & {85.1519 } &  {63.97m}  \\

        GAT \citep{kool2018attention}  & RL, G & {11.6096} & {8.3081 } & {5.03s} & {20.0188} & {20.9902 } & {1.51m} & {31.1526} & {34.7539 } & {3.18m}  \\

        GAT \citep{kool2018attention}  & RL, BS & {11.3769} & {6.1364 } & {5.77m} & {19.5283} & {18.0257 } & {21.99m} & {29.9048} & {29.2359 } & {1.64h}  \\

        GCN \citep{joshi2019efficient} & SL, G & {17.0141} & {58.7272 } &  {59.11s} & {29.7173} & {79.6063 } & {6.67m} & {48.6151} & {110.2900 } &  {28.52m}  \\

        GCN \citep{joshi2019efficient} & SL, BS & {16.1878} & {51.0185 } &  {4.63m} & {30.3702} & {83.5523 } &  {38.02m} & {51.2593} & {121.7278 } &  {51.67m}  \\

        GCN \citep{joshi2019efficient} & SL, BS* & {16.2081} & {51.2079 } & {3.97m} & {30.4258} & {83.8883 } & {30.62m} & {51.0992} & {121.0357 } & {3.23h}  \\

        \hline
        \multirow{2}{*} {Att-GCRN\citep{fu2021generalize}} & \multirow{2}{*}{\tabincell{c}{SL+RL \\MCTS}} & \multirow{2}{*}{{10.7358}} & \multirow{2}{*}{{0.1563 }} & {20.62s} +  & \multirow{2}{*}{16.7471} & \multirow{2}{*}{{1.2169 }} & {31.17s} +  & \multirow{2}{*}{{23.5153}} & \multirow{2}{*}{{1.7179 }} & {43.94s} +   \\
        & & & & 1.33m & & & 3.33m & & & 6.68m\\ \hline

        % \multirow{2}{*} {\tabincell{c}{Random Init ($T = 0.01$)}} & \multirow{2}{*}{MCTS} & \multirow{2}{*}{{NA}} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{NA} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{{7.8752}} & \multirow{2}{*}{1.473 } & {0+}   \\
        % & & & & NA & & & NA & & & 6m\\     \hline
        %  \multirow{2}{*} {\tabincell{c}{Random Init ($T = 0.02$)}} & \multirow{2}{*}{MCTS} & \multirow{2}{*}{{NA}} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{NA} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{{7.8483}} & \multirow{2}{*}{1.126 } & {0+}   \\
        % & & & & NA & & & NA & & & 12m\\     \hline
        %   \multirow{2}{*} {\tabincell{c}{Uniform Init ($T = 0.01$)}} & \multirow{2}{*}{MCTS} & \multirow{2}{*}{{NA}} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{NA} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{{7.8332}} & \multirow{2}{*}{0.932 } & {0+}   \\
        % & & & & NA & & & NA & & & 6m\\     \hline     
        %   \multirow{2}{*} {\tabincell{c}{Uniform Init ($T = 0.02$)}} & \multirow{2}{*}{MCTS} & \multirow{2}{*}{{NA}} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{NA} & \multirow{2}{*}{{NA}} & {NA} +  & \multirow{2}{*}{{7.8084}} & \multirow{2}{*}{0.612 } & {0+}   \\
        % & & & & NA & & & NA & & & 12m\\     \hline  
        
        \multirow{2}{*} {\textbf{UTSP (Ours)}} & \multirow{2}{*}{UL, Search} & \multirow{2}{*}{{10.7289}} & \multirow{2}{*}{\textbf{0.0918}} & {0.56m} +  & \multirow{2}{*}{16.6846} & \multirow{2}{*}{\textbf{0.8394}} & {1.37m} +  & \multirow{2}{*}{{23.3903}} & \multirow{2}{*}{\textbf{1.1770}} & {3.35m+}   \\
         & & & & 1.11m & & & 1.33m & & & 2.67m\\ 
         
        % \multirow{1}{*} {\textbf{Ours (Restart)} ($T = 0.04$s)} & \multirow{1}{*}{UL, Search} & \multirow{1}{*}{{10.7405}} & \multirow{1}{*}{\textbf{0.1996}} & {0.56m} +  & \multirow{1}{*}{16.6847} & \multirow{1}{*}{\textbf{0.8394}} & {1.37m} +  & \multirow{1}{*}{{23.3903}} & \multirow{1}{*}{\textbf{1.1770}} & {3.35m+}   \\
        %  & & & & 0.53m & & & 1.33m & & & 2.67m\\
\bottomrule
        % \bottomrule[2pt]
    \end{tabular}
\end{table*}
% \twocolumn

==> Tables/Tsp10kperformance.tex <==
\begin{table*}[t]
\footnotesize
\centering
\caption{Results of SAG + Local Search on TSP instances with 10,000 nodes.}
\label{table:largeinstance}
    \begin{tabular}{l|l|lll}
       \multirow{2}{*}{Method} & \multirow{2}{*}{Type}  & \multicolumn{3}{c}{TSP10000}\\
         &  & Length & Gap w.r.t. LKH3 (\%) & Time \\
        \hline
        LKH3 & Heuristic & 71.7778 & - & 8.8h \\
        \hline

        GAT \citep{kool2018attention} & RL, S & {431.5812} & {501.2737} & {12.63m}  \\
        GAT \citep{kool2018attention} & RL, G & {141.6846} & {97.3932} & {5.99m}    \\
        GAT \citep{kool2018attention} & RL, BS & {129.4012} & {80.2802} & {1.81h}   \\

        % \hline
        \multirow{2}{*}{Att-GCRN \citep{fu2021generalize}}  & \multirow{2}{*}{SL+RL+MCTS} & \multirow{2}{*}{74.2374} & \multirow{2}{*}{{3.4269}} & {4.16m} + \\
        & & & & 17.6m \\
        \hline
        \multirow{2}{*}{Ours}  & \multirow{2}{*}{UL, Search} & \multirow{2}{*}{73.9523} & \multirow{2}{*}{\textbf{3.0295}} & {7m} + \\
        & & & & 21m \\ 
        \bottomrule

    \end{tabular}
\end{table*}
